Sui Lutris: A Blockchain Combining Broadcast and Consensus

Sui Lutris is the first smart-contract platform to sustainably achieve sub-second finality. It achieves this significant decrease by employing consensusless agreement not only for simple payments but for a large variety of transactions. Unlike prior work, Sui Lutris neither compromises expressiveness nor throughput and can run perpetually without restarts. Sui Lutris achieves this by safely integrating consensuless agreement with a high-throughput consensus protocol that is invoked out of the critical finality path but ensures that when a transaction is at risk of inconsistent concurrent accesses, its settlement is delayed until the total ordering is resolved. Building such a hybrid architecture is especially delicate during reconfiguration events, where the system needs to preserve the safety of the consensusless path without compromising the long-term liveness of potentially misconfigured clients. We thus develop a novel reconfiguration protocol, the first to provably show the safe and efficient reconfiguration of a consensusless blockchain. Sui Lutris is currently running in production and underpins the Sui smart-contract platform. Combined with the use of Objects instead of accounts it enables the safe execution of smart contracts that expose objects as a first-class resource. In our experiments Sui Lutris achieves latency lower than 0.5 seconds for throughput up to 5,000 certificates per second (150k ops/s with transaction blocks), compared to the state-of-the-art real-world consensus latencies of 3 seconds. Furthermore, it gracefully handles validators crash-recovery and does not suffer visible performance degradation during reconfiguration.

==> sections/200Background.tex <==
\subsection{Background}
https://www.overleaf.com/project/62ed15672bd383721edd741e

==> sections/250Programming.tex <==
\section{\sysname smart contract programming} \label{sec:move}
\sysname smart contracts are written in the Move\cite{move_white} language. Move is safe and expressive, and its type system and data model naturally support the parallel agreement/execution strategies that make \sysname scalable.
Move is an open-source programming language for building smart contracts originally developed at Facebook for the Diem blockchain. The language is platform-agnostic, and in addition to being adopted by \sysname, it has been gaining popularity on other platforms (e.g., 0L, StarCoin). 

In this section we will discuss the main features of the Move language and explain how it is used to create and manage assets on \sysname. A more thorough explanation of Move's features can be found in the Move Programming Language book\footnote{\url{https://diem.github.io/move/}} and more \sysname-specific Move content can be found in the \sysname Developer Portal\footnote{\url{https://github.com/MystenLabs/fastnft/blob/main/doc/SUMMARY.md}}, and a more formal description of Move in the context of Sui can be found in Section~\ref{sec:model}.

%In traditional smart contract programming solutions, for example those used on the Ethereum platform (e.g., Solidity language), only one type of asset, typically a native coin (e.g., Eth), is directly supported in a smart contract language. This support includes a set of safety guarantees that help avoid common problems when managing assets, such as double-spending. At the same time, while custom assets, such as Non-Fungible Tokens (NFTs), can be created on these platforms, they will not enjoy the same level protection from programming mistakes, as they have no actual presence at the language level.

%On the other hand, Move has been designed to allow expressing assets as user-defined custom language-level data types that will enjoy the same level of protection as a native coin. In fact a native coin on a platform using the Move language has the same status as any other asset managed by the platform, all of which enjoy the same language-level guarantees.

%In Sui, both the concept of a coin and of any other asset managed by the platform, is expressed as an object defined as a custom \texttt{struct} type at the Move language level, akin to struct types used in other more traditional programming languages, such as C or C++\footnote{We simplify the examples to avoid muddying the discussion with Move language details, such as generic types, that are irrelevant at this point}:

\subsection{Overview}
\label{sec:move-overview}

\sysname's global state includes a pool of programmable objects created and managed by Move \emph{packages} that are collections of Move modules (see Section~\ref{sec:modules} for details) containing Move functions and types. Move packages themselves are also objects. Thus, \sysname objects can be partitioned into two categories:
\begin{itemize}
    \item \textbf{Struct data values}: Typed data governed by Move modules. Each object is a struct value with fields that can contain primitive types (e.g. integers, addresses), other objects, and non-object structs.
    \item \textbf{Package code values}: a set of related Move bytecode modules published as an atomic unit. Each module in a package can depend both on other modules in that package and on modules in previously published packages.
\end{itemize}

Objects can encode assets (e.g., fungible or non-fungible tokens), \emph{capabilities} granting the permission to call certain functions or create other objects, ``smart contracts'' that manage other assets, and so on--it's up to the programmer to decide. The Move code to declare a custom \sysname object type looks like this:
\begin{lstlisting}[basicstyle=\scriptsize\ttfamily,language=Move]
struct Obj has key {
  id: VersionedID, // globally unique ID and version
  f: u64 // objects can have primitive fields
  g: OtherObj // fields can also store other objects
}
\end{lstlisting}

All structs representing \sysname objects (but not all Move struct values) must have the \code{id} field and the \code{key} ability\footnote{\url{https://diem.github.io/move/abilities.html}} indicating that the value can be stored in \sysname's global object pool. 

\subsubsection{Modules}
\label{sec:modules}
A Move program is organized as a set of modules, each consisting of a list of struct declarations and function declarations. A module can import struct types from other modules and invoke functions declared by other modules. 

Values declared in one Move module can flow into another--e.g., module \code{OtherObj} in the example above could be defined in a different module than the module defining \code{Obj}. This is different from most smart contract languages, which allow only unstructured bytes to flow across contract boundaries. However, Move is able to support this because it provides encapsulation features to help programmers write \emph{robustly safe}~\cite{DBLP:journals/corr/abs-2110-05043} code. Specifically, Move's type system ensures that a type like \code{Obj} above can only be created, destroyed, copied, read, and written by functions inside the module that declares the type. This allows a module to enforce strong invariants on its declared types that continue to hold even when they flow across smart contract trust boundaries. 
%For example, if the functions inside the module \code{M} declaring \code{Obj} ensures that the field \code{f} is always nonzero, this property will continue to hold on \code{Obj}'s everywhere in the system.

\subsubsection{Transactions and Entrypoints.}
The global object pool is updated via transactions that can create, destroy, read, and write objects. A transaction must take each existing object it wishes to operate on as an input. In addition, a transaction must include the versioned ID of a package object, the name of a module and function inside that package, and arguments to the function (including input objects). For example, to call the function
%
\begin{lstlisting}[basicstyle=\scriptsize\ttfamily,language=Move]
public fun entrypoint(
  o1: Obj, o2: &mut Obj, o3: &Obj, x: u64, ctx: &mut TxContext
) { ... }
\end{lstlisting}
%
a transaction must supply ID's for three distinct objects whose type is \code{Obj} and an integer to bind to \code{x}. The \code{TxContext} is a special parameter filled in by the runtime that contains the sender address and information required to create new objects. 

Inputs to an entrypoint (and more generally, to any Move function) can be passed with different mutability permissions encoded in the type. An \code{Obj} input can be read, written, transferred, or destroyed. A \code{&mut Obj} input can only be read or written, and a \code{&Obj} can only be read. The transaction sender must be authorized to use each of the input objects with the specified mutability permissions--see Section~\ref{sec:owners} for more detail.

\subsubsection{Creating and Transferring Objects.}
Programmers can create objects by using the \code{TxContext} passed into the entrypoint to generate a fresh ID for the object:
\begin{lstlisting}[basicstyle=\scriptsize\ttfamily,language=Move]
public fun create_then_transfer(
  f: u64, g: OtherObj, o1: Obj, ctx: &mut TxContext
) {
  let o2 = Obj { id: TxContext::fresh_id(ctx), f, g };
  Transfer::transfer(o1, TxContext:sender());
  Transfer::transfer(o2, TxContext:sender());
}
\end{lstlisting}

This code takes two objects of type \code{OtherObj} and \code{Obj} as input, uses the first one and the generated ID to create a new \code{Obj}, and then transfers both \code{Obj} objects to the transaction sender. Once an object has been transferred, it flows into the global object pool and cannot be accessed by code in the remainder of the transaction. The \code{Transfer} module is part of the \code{Sui} standard library, which includes functions for transferring objects to user addresses and to other objects.

We note that if the programmer code neglected to include one of the \code{transfer} calls, this code would be rejected by the Move type system. Move enforces \emph{resource safety}~\cite{DBLP:journals/corr/abs-2004-05106} protections to ensure that objects cannot be created without permission, copied, or accidentally destroyed. Another example of resource safety would be an attempt to transfer the same object twice, which would also be rejected by the Move type system.



==> sections/270ProgrammingModel.tex <==
\section{The \sysname programming model} \label{sec:model}

In this section, we expand on the informal description of the Sui programming model from Section \ref{sec:move} by presenting detailed semantic definitions. The previous section showed examples of Move source code; here we define the structure of Move bytecode. Developers write, test, and formally verify~\cite{DBLP:journals/corr/abs-2110-08362, DBLP:conf/cav/ZhongCQGBPZBD20} Move source code locally, then compile it to Move bytecode before publishing it to the blockchain. Any Move bytecode be published on-chain must pass through a \emph{bytecode verifier}\cite{move_white, DBLP:journals/corr/abs-2004-05106} to ensure that it satisfies key properties such as type, memory, and resource safety.

As mentioned in Section~\ref{sec:move}, Move is a platform-agnostic language which can be adapted to fit specific needs of different systems without forking the core language. In the following description, we define both concepts from core Move language (denoted in black text) and Sui-specific features extending the core Move language (denoted with \suimove{orange} text). 
%For simplicity, we define the Sui features as if they were part of the Move bytecode language, but at the implementation level we have added these features via a Sui adapter, native functions, and framework modules.

\subsection{Modules}
\label{sec:mod-pkg}

\begin{table}[H]
  \begin{tabular}{|ll|}
  \hline
  $\Module =$ & $\ModuleName \times$ \\
  & $(\StructName \pfun \StructDecl) \times$ \\
  & $(\ProcName \pfun \ProcDecl) \times \suimove{\ProcDecl}$ \\
  $\mathsf{\GenParam} =$ & $\seq{\mathsf{Ability}}$ \\
  $\StructDecl =$ & $(\FieldName \pfun \StoreableType) \times$ \\
  & $\seq{\mathsf{Ability}} \times \seq{\mathsf{\GenParam}}$ \\
  $\ProcDecl$ = & $\seq{\Type} \seq{\Type} \times \seq{\Instruction} \times \seq{\mathsf{\GenParam}}$ \\
  $\Instruction=$ & $\suimove{\mathsf{TransferToAddr}} ~|~ \suimove{\mathsf{TransferToObj}} ~|~ \suimove{\mathsf{ShareMut}} ~|~$ \\
  & $\suimove{\mathsf{ShareImmut}} ~|~ \ldots$ \\
    \hline
 \end{tabular}
 \caption{Module}
 \label{tab:mod-pkg}
\end{table}

Move code is organized into \emph{modules} whose structure is defined in Table~\ref{tab:mod-pkg}. A module consists of a collection of named \emph{struct} declarations and a collection of named \emph{function} declarations (examples of these declaration are provided in Section~\ref{sec:move-overview}). A module also contains a special function declaration serving as the module \emph{initializer}. This function is invoked exactly once at the time the module is published on-chain.

A struct declaration is a collection of named fields, where a field name is mapped to a storeable type. Its declaration also includes an optional list of abilities (see Section~\ref{tab:types-abilities} for a description of storeable types and abilities). A struct declaration may also include a list of \emph{generic parameters} with ability constraints, in which case we call it a \emph{generic struct} declaration, for example \code{struct Wrapper<T: copy>\{ t: T \}}. A generic parameter represents a type to be used when declaring struct fields -- it is unknown at the time of struct declaration, with a  \emph{concrete} type provided when the struct is instantiated (i.e., as struct value is created).

A function declaration includes a list of parameter types, a list of return types, and a list of instructions forming the function's body. A function declaration may also include a list of generic parameters with ability constraints, in which case we call it a \emph{generic function} declaration, for example \code{fun unwrap<T: copy>(p: Wrapper<T>)\{\}}. Similarly to struct declarations, a generic parameter represents a type unknown at function declaration time, but which is nevertheless used when declaring function parameters, return values and a function body (concrete type is provided when a function is called).

Instructions that can appear in a function body include all ordinary Move instructions with the exception of global storage instructions (e.g., \code{move_to}, \code{move_from}, \code{borrow_global}). See \cite{DBLP:journals/corr/abs-2110-05043} for a complete list of core Move's instructions and their semantics. In Sui persistent storage is supported via Sui's global object pool rather than the account-based global storage of core Move. 

There are four Sui-specific object operations. Each of these operations changes the ownership metadata of the object (see Section \ref{sec:objects}) and returns it to the global object pool. Most simply, a Sui object can be transferred to the address of a Sui end-user. An object can also be transferred to another \emph{parent} object--this operation requires the caller to supply a mutable reference to the parent object in addition to the child object. An object can be mutably \emph{shared} so it can be read/written by anyone in the Sui system. Finally, an object can be immutably shared so it can be read by anyone in the Sui system, but not written by anyone.

The ability to distinguish between different kinds of ownership is a unique feature of Sui. In other blockchain platforms we are aware of, every contract and object is mutably shared. As we will explain in Section~\ref{sec:system}, Sui leverages this information for parallel transaction execution (for all transactions) and parallel agreement (for transactions involving objects without shared mutability).

\subsection{Types and Abilities}

\begin{table}[H]
  \begin{tabular}{|ll|}
  \hline
  $\GroundType =$ & $\set{\texttt{address}, \suimove{\texttt{id}}, \texttt{bool}, \texttt{u8}, \texttt{u64}, \ldots}$ \\
  $\StructType =$ & $\ModuleName \times \StructName \times$  \\
  & $\seq{\StoreableType}$ \\
  $\StoreableType =$ & $\GroundType \uplus \StructType \uplus$\\
  & $\TypeArg \uplus \VecType$ \\
  $\VecType =$ & $\StoreableType$ \\
  $\TypeArg =$ & $\mathbb{N}$ \\
  $\MutabilityQual =$ & $\set{\texttt{mut}, \texttt{immut}}$ \\
  $\ReferenceType =$ & $\StoreableType \times \MutabilityQual$ \\
  $\Type =$ & $\mathsf{ReferenceType} \uplus \StoreableType$ \\
  $\mathsf{Ability} =$ & $\set{\texttt{key}, \texttt{store}, \texttt{copy}, \texttt{drop}}$ \\
  \hline
  \end{tabular}
 \caption{Types and Abilities}
 \label{tab:types-abilities}
\end{table}

A Move program manipulates both data stored in Sui global object pool and transient data created when the Move program executes. Both objects and transient data are Move \emph{values} at the language level. However, not all values are created equal -- they may have different properties and different structure as prescribed by their types. 

The types used in Move are defined in Table~\ref{tab:types-abilities}. Move supports many of the same \emph{primitive types} supported in other programming languages, such as a boolean type or unsigned integer types of various sizes. In addition, core Move has an \code{address} type representing an end-user in the system that is also used to identify the sender of a transaction and (in Sui) the owner of an object. Finally, Sui defines an \code{id} type representing an identity of a Sui object-- see Section~\ref{sec:objects} for details.

A \emph{struct type} describes an instance (i.e., a value) of a struct declared in a given module (see Section~\ref{sec:mod-pkg} for information on struct declarations). A struct type representing a generic struct declaration (i.e., \emph{generic struct} type) includes a list of \emph{storeable types} -- this list is the counterpart of the generic parameter list in the struct declaration. A storeable type can be either a \emph{concrete type} (a primitive or a struct) or a \emph{generic type}. We call such types storeable because they can appear as fields of structs and in objects stored persistently on-chain, whereas reference types cannot.

For example, the \code{Wrapper<u64>} struct type is a generic struct type parameterized with a concrete (primitive) storeable type \code{u64} -- this kind of type can be used to create a struct instance (i.e.,value). On the other hand, the same generic struct type can be parameterized with a generic type (e.g., \code{struct Parent<T> \{ w: Wrapper<T> \}}) coming from a generic parameter of the enclosing struct or function declaration  -- this kind of type can be used to declare struct fields, function params, etc. Structurally, a generic type is an integer index (defined as $\mathbb{N}$ in Table~\ref{tab:txn}) into the list of generic parameters in the enclosing struct or function declaration.

A \emph{vector type} in Move describes a variable length collection of homogenous values. A Move vector can only contain storeable types, and it is also a storeable type itself.

A Move program can operate directly on values or access them indirectly via references. A \emph{reference type} includes both the storeable type referenced and a \emph{mutability qualifier} used to determine (and enforce) whether a value of a given type can be read and written (\texttt{mut}) or only read (\texttt{immut}). Consequently, the most general form of a Move value type (\code{Type} in Table~\ref{tab:types-abilities}) can be either a storeable type or a reference type.

Finally, \emph{abilities} in Move control what actions are permissible for values of a given type, such as whether a value of a given type can be copied (duplicated). Abilities constraint struct declarations and generic type parameters. The Move bytecode verifier is responsible for ensuring that sensitive operations like copies can only be performed on types with the corresponding ability.

\subsection{Objects and Ownership}
\label{sec:objects}

\begin{table}[H]
  \begin{tabular}{|ll|}
  \hline
  $\transactiondigest =$ & $Com(\transaction)$ \\
  $\objectid =$ & $Com(\transactiondigest \times \mathbb{N})$ \\
  $\mathsf{SingleOwner} =$ & $\AccountAddress \uplus \objectid$ \\
  $\mathsf{Shared} =$ & $\set{\texttt{shared\_mut}, \texttt{shared\_immut}}$ \\
  $\mathsf{Ownership} =$ & $\mathsf{SingleOwner} \uplus \mathsf{Shared}$ \\
  $\mathsf{StructObj} =$ & $\StructType \times \Struct$ \\
  $\mathsf{ObjContents} =$ & $\mathsf{StructObj} \uplus \mathsf{Package}$ \\
  $\Object =$ & $\mathsf{ObjContents} \times \objectid \times \mathsf{Ownership} \times \Version$ \\
  \hline
 \end{tabular}
 \caption{Objects and Ownership}
 \label{tab:objects-ownership}
\end{table}

 Each Sui object has a globally unique identifier ($\objectid$ in Table~\ref{tab:objects-ownership}) that serves as the persistent identity of the object as it flows between owners and into and out of other objects.
 This ID is assigned to the object by the transaction that creates it.
 An object ID is created by applying a collision-resistant hash function to the contents of the current transaction and to a counter recording how many objects the transaction has created. 
 A transaction (and thus its digest) is guaranteed to be unique due to constraints on the input objects of the transaction, as we will explain subsequently.
 
 In addition to an ID, each object carries metadata about its ownership. An object is either uniquely owned by an address or another object, shared with write/read permissions, or shared with only read permissions. The ownership of an object determines whether and how a transaction can use it as an input. Broadly, a uniquely owned object can only be used in a transaction initiated by its owner or including its parent object as an input, whereas a shared object can be used by any transaction, but only with the specified mutability permissions. See Section \ref{sec:owners} for a full explanation.
 
 There are two types of objects: package code objects, and struct data objects. A package object contains of a list of modules. A struct object contains a Move struct value and the Move type of that value. The contents of an object may change, but its ID, object type (package vs struct) and Move struct type are immutable. This ensures that objects are strongly typed and have a persistent identity.
 
 Finally, an object contains a version. Freshly created objects have version 0, and an object's version is incremented each time a transaction takes the object as an input.

\subsection{Addresses and Authenticators}
\label{sec:address}

\begin{table}[H]
  \begin{tabular}{|ll|}
  \hline
  $\Authenticator =$ & $\mathsf{Ed25519PubKey} \uplus \mathsf{ECDSAPubKey} \uplus \ldots$ \\
  $\AccountAddress =$ & $Com(\Authenticator)$ \\
  \hline
 \end{tabular}
 \caption{Addresses and Authenticators}
 \label{tab:addr-authenticator}
\end{table}

 An address is the persistent identity of a Sui end-user (although note that a single user can have an arbitrary number of addresses). To transfer an object to another user, the sender must know the address of the recipient.

As we will discuss shortly, a Sui transaction must contain the address of the user sending (i.e., initiating) the transaction and an \emph{authenticator} whose digest matches the address. The separation between addresses and authenticators enables \emph{cryptographic agility}. An authenticator can be a public key from any signature scheme, even if the schemes use different key lengths (e.g., to support post-quantum signatures). In addition, an authenticator need not be a single public key--it could also be (e.g.) a K-of-N multisig key. 
 
\subsection{Transactions}
 
\begin{table}[H]
  \begin{tabular}{|ll|}
  \hline
  $\ObjRef=$ & $\objectid \times \Version \times Com(\Object)$ \\
  $\textsf{CallTarget}=$ & $\ObjRef \times \ModuleName \times \ProcName$ \\
  $\textsf{CallArg}=$ & $\ObjRef \uplus \objectid \uplus \GroundType$ \\
  $\mathsf{Package} =$ & $\seq{\Module}$ \\
  $\textsf{Publish}=$ & $\mathsf{Package} \times \seq{\ObjRef}$ \\
  $\textsf{Call} =$ & $\textsf{CallTarget} \times \seq{\StoreableType} \times \seq{\mathsf{CallArg}}$ \\
  $\mathsf{GasInfo} =$ & $\ObjRef \times \textsf{MaxGas} \times \textsf{BaseFee} \times \textsf{Tip}$ \\
  $\mathsf{Tx} =$ & $(\textsf{Call} \uplus \textsf{Publish}) \times \mathsf{GasInfo} \times \mathsf{Addr} \times \mathsf{Authenticator}$ \\ 
  \hline 
  \end{tabular}
  \caption{Transactions}
  \label{tab:txn}
\end{table}

Sui has two different transaction types: publishing a new Move package, and calling a previously published Move package. A publish transaction contains a \emph{package}--a set of modules that will be published together as a single object, as well as the dependencies of all the modules in this package (encoded as a list of object references that must refer to already-published package objects). To execute a publish transaction, the Sui runtime will run the Move bytecode verifier on each package, link the package against its dependencies, and run the module initializer of each module. Module initializers are useful for bootstrapping the initial state of an application implemented by the package.

A call transaction's most important arguments are object inputs. Object arguments are either specified via an object reference (for single-owner and shared immutable objects) or an object ID (for shared mutable objects). An object reference consists of an object ID, an object version, and the hash of the object value. The Sui runtime will resolve both object ID's and object references to object values stored in the global object pool. For object references, the runtime will check the version of the reference against the version of the object in the pool, as well as checking that the reference's hash matches the pool object. This ensures that the runtime's view of the object matches the transaction sender's view of the object.

In addition, a call transaction accepts type arguments and pure value arguments. Type arguments instantiate generic type parameters of the entrypoint function to be invoked (e.g., if the entrypoint function is \code{send_coin<T>(c: Coin<T>, ...)}, the generic type parameter \code{T} could be instantiated with the type argument \code{SUI} to send the Sui native token). Pure values can include primitive types and vectors of primitive types, but not struct types. 

The function to be invoked by the call is specified via an object reference (which must refer to a package object), a name of a module in that package, and a name of a function in that package. To execute a call transaction, the Sui runtime will resolve the function, bind the type, object, and value arguments to the function parameters, and use the Move VM to execute the function.

Both call and publish transactions are subject to gas metering and gas fees. The metering limit is expressed by a maximum gas budget. The runtime will execute the transaction until the budget is reached, and will abort with no effects (other than deducting fees and reporting the abort code) if the budget is exhausted.

The fees are deducted from a \emph{gas object} specified as an object reference. This object must be a Sui native token (i.e., its type must be \code{Coin<SUI>}). Sui uses EIP1559\footnote{\url{https://github.com/ethereum/EIPs/blob/master/EIPS/eip-1559.md}}-style fees: the protocol defines a base fee (denominated in gas units per Sui token) that is algorithmically adjusted at epoch boundaries, and the transaction sender can also include an optional tip (denominated in Sui tokens). Under normal system load, transactions will be processed promptly even with no tip. However, if the system is congested, transactions with a larger tip will be prioritized. The total fee deduced from the gas object is $(\mathsf{GasUsed} * \mathsf{BaseFee}) + \mathsf{Tip}$.

\subsection{Transaction Effects}

\begin{table}[H]
  \begin{tabular}{|ll|}
  \hline
   $\mathsf{Event} =$ & $\StructType \times \Struct$ \\
   $\mathsf{Create} =$ & $\Object$ \\
   $\mathsf{Update} =$ & $\Object$ \\
   $\mathsf{Wrap} =$ & $\objectid \times \Version$ \\
   $\mathsf{Delete} =$ & $\objectid \times \Version$ \\
   $\mathsf{ObjEffect} =$ & $\mathsf{Create} \uplus \mathsf{Update} \uplus \mathsf{Wrap} \uplus \mathsf{Delete}$ \\
   $\mathsf{AbortCode} =$ & $\mathbb{N} \times \ModuleName$ \\
   $\mathsf{SuccessEffects} =$ & $\seq{\mathsf{ObjEffect}} \times \seq{\mathsf{Event}}$ \\
   $\mathsf{AbortEffects} =$ & $\mathsf{AbortCode}$ \\
   $\mathsf{TxEffects} =$ & $\mathsf{SuccessEffects} \uplus \mathsf{AbortEffects}$ \\
   \hline
  \end{tabular}
  \caption{Transaction Effects}
  \label{tab:effect}
\end{table}

Transaction execution generates transaction effects which are different in the case when execution of a transaction is successful (\code{SuccessEffects} in Table~\ref{tab:effect}) and when it is not (\code{AbortEffects} in Table~\ref{tab:effect}).

Upon successful transaction execution, transaction effects include information about  changes made to Sui's global object pool (including both updates to existing objects and freshly created objects) and \emph{events} generated during transaction execution. Another effect of successful transaction execution could be object removal (i.e., deletion) from the global pool and also wrapping (i.e., embedding) one object into another, which has a similar effect to removal -- a wrapped object disappears from the global pool and exists only as a part of the object that wraps it. Since deleted and wrapped objects are no longer accessible in the global pool, these effects are represented by the ID and version of the object.

Events encode side effects of successful transaction execution beyond updates to the global object pool. Structurally, an event consists of a Move struct and its type. Events are intended to be consumed by actors outside the blockchain, but cannot be read by Move programs.

Transactions in Move have an all-or-nothing semantics -- if execution of a transaction aborts at some point (e.g., due to an unexpected failure), even if some changes to objects had happened (or some events had been generated) prior to this point, none of these effects persist in an aborted transaction. Instead, an aborted transaction effect includes a numeric abort code and the name of a module where the transaction abort occurred. Gas fees are still charged for aborted transactions.

==> sections/310Checkpoints.tex <==
\section{Checkpoints} \label{sec:checkpoint}
% \sysname combines two modes: one by which transactions on owned objects are executed asynchronously via reliable broadcast, and one by which transactions on shared objects acquire locks through a consensus algorithm. Both modes lead to transaction finality upon completion. As a result, the state of replicas is composed of the set of processed owned object transactions and the sequence number of shared object transactions. While two honest replicas are consistent, it is expensive to compare their states since there may be no point at which they are equal, and determining the set difference is expensive.

%The \sysname checkpoint protocol aims to be particularly efficient in creating checkpoints. The construction of a checkpoint that contains $\mathcal{O}(K)$ new transactions should on average cost $\mathcal{O}(k), k \ll K$ in communication for each Node (abusing O-notation). This is particularly true if nodes are largely in sync with each other’s state, and only need to largely confirm they are in agreement or only download a small set of transactions to agree.
%
%Furthermore, most checkpoints (except the end of epoch one) are constructed while newer transactions are being processed by validators. The checkpoint construction process should involve no service interruption or degradation.

%\subsection{Purpose}  \label{sec:checkpoint-properties}

\george{NOTE: we will be re-writing this section once we have worked out the latest checkpoint scheme.}

Checkpoints provide a sequence of transaction sets that a quorum of validators agrees upon as having been executed within the Sui system. These sets are then stored by a quorum of validators ensuring availability of both the transactions and effects of transactions for anyone (including lagging validators, full nodes, and light clients, see \Cref{sec:ecosystem}) to download. They are produced regularly over time, e.g., every 10 minutes.
%
Checkpoints are necessary for some use cases and desirable for others.
\begin{itemize}
    \item \textbf{Reconfiguration:} A simple epoch change and reconfiguration protocol (see \Cref{sec:reconfiguration}) advances the epoch at a boundary of a well-defined checkpoint\footnote{While a reconfiguration algorithm may exist without requiring such checkpoints we do not know of a practical one.}. Reconfiguration ensures that the contents of the last checkpoint are carried over to the new epoch and that updates not in a checkpoint are discarded at the start of the new epoch.
          If a transaction reaches finality in an epoch, \sysname needs to ensure that it is contained in a checkpoint before the end of the epoch.

    \item \textbf{Bootstrapping and synchronization:} The sequence of checkpoints may also be used for synchronization by full nodes (see \Cref{sec:ecosystem}) to bundle updates of the state, and download it to update lagging, recovering, or fresh validators efficiently.

    \item \textbf{Audit \& light clients:} Checkpoints are also desirable for various forms of bookkeeping after transactions reach finality. Each checkpoint contains an authenticated data structure (such as a Merkle tree~\cite{merkle1979secrecy} root) committing to all transactions or objects in the database. This allows \sysname to support light client protocols (see \Cref{sec:ecosystem}) that require totality (i.e., a guarantee that all the state or transactions up to a point are known), such as audits.
\end{itemize}
%
\sysname differs from other blockchains in that it constructs checkpoints after transaction execution and finalization, to reduce the latency impact on the transaction execution path.

% \para{Checkpoint properties}
% \sysname checkpoints achieve the standard security properties below: \begin{itemize}
%     \item \textbf{Safety:} Each checkpoint should contain (directly or indirectly) all transactions that have been `previously' finalized in the system. This means that if a transaction's certificate is processed by a quorum at time $t$ and then a checkpoint construction occurs at time $t' > t$, the checkpoint at $t'$ should contain the transaction.
%     \item \textbf{Liveness:} Each checkpoint should represent some progress over the state in a previous checkpoint, i.e., at least one new transaction should be contained within each new checkpoint.
% \end{itemize}

\subsection{Spanning Tree Checkpoint Creation} \label{sec:checkpoint-protocol}

A trivial design to produce checkpoints would be for each validator to publish their local checkpoint proposal on chain and take the union of the first 2f+1 such proposals as the next checkpoint. This requires re-sharing large sets of transactions that other validators largely already hold. We design the \sysname checkpoint mechanism to minimize the amount of data that needs to be re-shared and sequenced, under the (credible) assumption that in most cases replicas largely have overlapping sets of processed transactions. Since checkpoints need to be identical between replicas they imply the use of an agreement protocol (consensus) to determine them. We use such a consensus protocol to sequence messages as a black box (see \Cref{sec:overview}):

%\para{Straw-man design}
%The process of creating checkpoints should be efficient in terms of minimizing the number of messages and their size, that need to be sequenced through consensus. A straw-man design would have all validators sequencing all transactions they process using a consensus algorithm (including the ones on owned objects that do not require sequencing). Periodically, each validator would also sequence a signal that the checkpoint boundary $i$ has been reached. All observers of the common sequence would await the first $2f+1$ such valid signals for each checkpoint $i$, then take all sequenced transactions not contained in a previous checkpoint, topologically sort them, and form a new checkpoint at that boundary.
%
%This approach is simple but has numerous efficiency downsides. (i) It requires all certificates processed by all validators to be sequenced, potentially multiple times, including certificates that would not need to be sequenced otherwise. (ii) It does not attempt the leverage the fact that two honest validators have sets of transactions that largely overlap. (iii) This approach also uses continuously the consensus algorithm and therefore requires a very high throughput implementation.
%
%\para{Spanning Tree Checkpoint Creation}
% The process, we call \emph{Spanning Tree Checkpoint}, proceeds in multiple steps.

\para{Step 1: Proposals}
Each validator signs a \emph{checkpoint proposal} message containing several transaction digests and effect digests pairs to be included in the next checkpoint. Honest proposals are complete, as in they contain all transaction dependencies necessary for all transactions to be executed; and extend the previous checkpoint. Each proposal has a signed header with an additive homomorphic hash of the contents of the pairs included~\cite{maitin2017elliptic}.

\para{Step 2: Compute fragments}
Validators download some proposals from other validators and construct one or more \emph{checkpoint fragments} representing their difference. Each fragment ``connects'' two proposals; it includes the signed homomorphic hashes of two validators and the list of actual certificates (not just digests) that are different across them. Note that given the elements of the sets representing the difference, it is possible to show the differences correspond to the signed homomorphic hashes included.

\para{Step 3: Fragments agreement}
As fragments are computed on each validator they are submitted to the consensus protocol by one of the two validators they `connect'. All validators observe a common sequence of fragments output by consensus. Invalid fragments are ignored by all, when signatures do not check, they contain the wrong sequence number, or shared object transactions that have not yet been sequenced.

\para{Step 4: Checkpoint creation}
Each validator attempts to reconstruct a checkpoint by combining fragments in the order they appear in the consensus output sequence. Specifically, a validator constructs the graph with validators as vertices and valid available fragments as edges, by adding fragments in the sequence as they are received. Inconsistent fragments from a single validator lead to an edge being ignored. When that graph contains a connected component of $2f+1$ validator vertices the checkpoint construction ends. The checkpoint will ultimately contain the union of the set of proposals of the validators represented as vertices in these connected components. Since the graph for each checkpoint starts initially empty and is augmented by all validators using the same sequence of fragments deterministically, the resulting connected component will be identical across honest validators.

If a validator observing the connected component is also a validator within the connected component, they have all the information necessary to compute the checkpoint: they take the union of their proposal and the sets of differences in all fragments representing edges in the connected components. Then they refine this set in various ways: (i) they remove any certificate for which the causal history is not included in the set; and (ii) order the set into a list following a deterministic topological order. Then they sign the resulting list of certificates and effects as the new \emph{signed checkpoint}. An authenticated data structure, such as roots of Merkle Trees~\cite{merkle1979secrecy} is also included, in the checkpoint to enable light client authenticated reads concerning the full state up to the checkpoint\footnote{Such reads are distinct from the light-client reads back by effects certificates, in that they can answer `not-in` queries that require an authenticated structure over a complete state, which is not monotonic~\cite{hellerstein2020keeping} and implies the need for agreement among replicas.}.

\para{Step 5: Checkpoint certificate}
Validators request the signed checkpoint metadata from all other validators. For those validators that cannot reconstruct the checkpoint contents, they may also request the contents of the checkpoint or use their proposal with a set reconciliation algorithm to efficiently recover the difference. A checkpoint with signatures of $f+1$ validators is considered valid and is called \emph{certified checkpoint}.

% \subsection{Checkpoint Messages}
% \george{Do we need this?}
% \sysname validators run the checkpoint protocol described in \Cref{sec:checkpoint-overview} by exchanging the following messages.

% \para{Checkpoint proposal}
% A \emph{checkpoint proposal} created by validator $a$ is defined as
% $$P_{a,i} = [\bar{T}_{a,i}, i, h^{+}(\bar{T}_{a,i})], \mathit{Sign}_{a}(i, h^{+}(\bar{T}_{a,i}))$$
% and contains the following fields:
% \begin{itemize}
%     \item A list of transactions $\bar{T}_{a, i}$ including the owner signature, but excluding any authority signatures from a certificate. Honest proposals are complete, as in they contain all transaction dependencies necessary for all transactions to be executed.
%     \item A sequence number $i$, starting at $i=0$ and monotonically increasing over the lifetime of the system.
%     \item An additive homomorphic hash of its contents $h^{+}(\bar{T}_{a,i})$.
%     \item A signature $\mathit{Sign}_{a}$ from the validator $a$ that created it.
% \end{itemize}

% \para{Checkpoint fragment}
% A \emph{checkpoint fragment} connecting the proposals of validators $a$ and $a'$ is defined as
% $$ F_{a, a', i} = [h^{+}(\bar{T}_{a,i}), h^{+}(\bar{T}_{a',i}), S_{a-a'}, S_{a'-a}]$$
% and contains the following fields:
% \begin{itemize}
%     \item The signed homomorphic hashes $h^{+}(\bar{T}_{a,i})$ and $h^{+}(\bar{T}_{a',i})$ of validators $a$ and $a'$.
%     \item The list of actual certificates (not just their digests) $S_{a-a'}$ and $S_{a'-a}$ that are different across the homomorphic hashes, namely $(\bar{T}_{a,i} - \bar{T}_{a',i})$ and $(\bar{T}_{a',i} - \bar{T}_{a,i})$. Note that given the elements of the sets representing the difference, it is possible to show the differences correspond to the signed homophobic hashes included.
% \end{itemize}

% \para{Certified checkpoint}
% A \emph{certified Checkpoint} is defined as
% $$C_i = [\bar{T}_i, i, h(C_{i-1})], \textit{Sign}_{\bar{A}}(C_i)$$
% and contains the following fields:
% \begin{itemize}
%     \item A list of transactions $\bar{T}_i$ including the owner signature, but excluding any authority signatures from a certificate. Each transaction is represented as its digest and the digest of its execution digest. They are sorted in topological order of execution.
%     \item The checkpoint sequence number $i$
%     \item the hash of the previous checkpoint $h(C_{i-1})$.
%     \item A set of $f+1$ signature $\textit{Sign}_{\bar{A}}(C_i)$ implicitly linking the checkpoint to an epoch.
% \end{itemize}

% \para{Signed checkpoint}
% A \emph{Signed checkpoint} contains the same information as a \emph{certified checkpoint} but is only signed by a single validator.

% \subsection{The \sysname Checkpoint Protocol}
% \alberto{Remove it; no need to stores for that}
% \todo{Explain (i) the extra stores that are needed to support checkpoints, (ii) what the validator does upon receiving each protocol message described in \Cref{sec:checkpoint-overview}.}

\subsection{Protocol Efficiency}
The \sysname checkpoint protocol can be efficiently implemented to further reduce the communication cost of creating checkpoint fragments and signed checkpoints.

\para{Efficient fragments creation}
Checkpoint fragments contain a list of certificates that is in the length of the \emph{difference} of the sets between validators in each fragment, and which becomes proportionately smaller as compared to the size of the proposal sets as sets become bigger when validators employ any best effort synchronization mechanism (such as the gossip protocol described in \Cref{sec:gossip}).
%The most straightforward implementation for constructing fragments involves validators downloading the full list of transactions and effect digests in other validator proposals. 
Efficient algorithms may be used to compute set differences for fragments such as Merkle Trees based reconciliation Trees~\cite{byers2002fast} or Invertible Bloom lookup tables (IBLT)~\cite{goodrich2011invertible}. These require bandwidth only in the order of the set difference size.

\para{Efficient signed checkpoint creation}
% Similar techniques may be used by validators that cannot reconstruct the checkpoint (as their proposal is not included in the checkpoint) to recover the checkpoint. Either by directly recovering the missing elements between the checkpoint and their checkpoint proposal or by using fragments with proposals in the checkpoint to recover the full contents of the checkpoint.
%
If a validator proposal is not included in the checkpoint, a validator making this proposal that knows a fragment (also not included) connecting itself to a validator with a proposal in the checkpoint also has all information necessary to reconstruct the checkpoint. The mean number of fragments that are necessary per validator to get a checkpoint is constant: as the number of edges in the graph including each validator increases, the probability that the graph is connected and contains a massive component increases exponentially with each additional link. Therefore as few as 3-4 fragments per validator are likely to be necessary even for large graphs.

% Optimizations to this process could include an adaptive strategy, in which validators pick other validators to make fragments informed by the fragments already sequenced to increase the size of the largest component to above $>2/3$ of take. However, another optimization objective could instead have honest validators pick fragments to sequence that are of minimal size, i.e., with other validators with transaction sets that are nearly identical, to minimize the size of fragments.



==> sections/322Sync.tex <==
\section{Validators Synchronization} \label{sec:sync}
Due to client failures or non-byzantine (crash) validator failures, some validators may not have processed all certificates. As a result causally related transactions depending on missing objects generated by these certificates would be rejected.

%\subsection{Relayers}
A client or external service, called a \emph{relayer}, can always update an honest validator to the point where it can process a correct transaction. It may do this using its store of past certificates, or using one or more other honest validators as a source for past certificates.
They are untrusted in terms of integrity, and their operation is keyless. Besides relayers, validators can run the relayer logic themselves to update each other.

\para{Synchronization protocol}
Given a certificate $c$ and a $\certdb$ store that includes $c$ and its causal history, a relayer can update an honest validator $v'$ to the point where $c$ would also be successfully executed.
This involves finding the smallest set of certificates unknown to $v'$ such that when processed the $\objdb$ store of $v'$ includes all inputs of $c$.
Updating a lagging validator $v'$ using a store $\certdb$ including the certificate $\cert$ involves the following process:
\begin{itemize}[leftmargin=*]
    \item The relayer maintains a list of certificates to synchronize (initially set to contain just $\cert$).
    \item The relayer considers the last $\cert$ requiring sync. It extracts the $\transaction$ within the $\cert$ and derives all its input objects (e.g., using $\txinput(\transaction)$).
    \item For each input object it checks whether the last $\transaction$ that generated or mutated objects (using the $Ct$ store) has a certificate within $v'$, otherwise its certificate is read from $Ct$ and added to the list of certificates to sync.
    \item If no more certificates can be added to the list (because no more inputs are missing from $v'$) the certificate list is sorted in a causal order and submitted to $v'$.
\end{itemize}
The algorithm above also applies to updating an object to a specific version to enable a new transaction. In this case, the certificate for the $\transaction$ that generated the object version, found in $\syncdb[\objectref]$, is submitted to the lagging validator. Once it is executed on $v'$ the object at the correct version will become available to use.

==> sections/350SmartContracts.tex <==
\section{Smart Contracts Programming}
\todo{This section is just fluff to say that Sui runs Move. @George would you like to handle it. I am not even sure we need.}


==> sections/360Ecosystem.tex <==
\section{The \sysname Ecosystem} \label{sec:ecosystem}
Aside from validators, the \sysname ecosystem includes a number of actors running client-side operations and facilitating the execution of the core protocol.

\para{Full Clients \& Replicas} 
Replicas, also sometimes called \emph{full clients} or \emph{full nodes}, do not validate new transactions, but maintain a consistent copy of the valid state of the system for the purposes of audit, as well as to construct transactions or operate services including read infrastructures for light client queries. Replicas can also help the validators to remain in sync by running the synchronization protocol described in \Cref{sec:sync}. Future validators start by running a replica before taking over validator operations (see \Cref{sec:reconfiguration}). \kostas{what about sparse nodes?}

%\para{Light Clients}
%\todo{Explain here all the facilities to help light clients and high-integrity reads: Lamport timestamps, certificate effects that are self-authenticating. Explain what finality means for clients and how a client finds out the latest state of an object if it only has its $\objectid$.}












%Both object references and transactions contain information that allows the authentication of the full causal chain of transactions that leads up to their creation or execution. Specifically, an object reference (\objectref) contains an \objectdigest\xspace that is an authenticator for the full state of the object, including the facility to get $\parent{\object}$, namely the \transactiondigest\xspace that created the object. Similarly, a \transactiondigest\xspace  authenticates a transaction, including the facility to extract through $\txinputs{\transaction}$ the object references of the input objects. Therefore the set of objects and certificates form a bipartite graph that is self-authenticating. Furthermore, effects structures are also signed, and may be collated into effects certificates that directly certify the results of transaction executions.

%These facilities may be used to support \emph{light clients} that can perform high-integrity reads into the state of \sysname, without maintaining a full replica node. Specifically an authority or full node may provide a succinct bundle of evidence, comprising a certificate $\cert$ on a transaction $\transaction $ and the input objects $[\Object]$ corresponding to $\txinputs{\transaction}$ to convince a light client that a transition can take place within \sysname. A light client may then submit this certificate, or check whether it has been seen by a quorum or sample of authorities to ensure finality. Or it may craft a transaction using the objects resulting from the execution, and observe whether it is successful.

%More directly, a service may provide an effects certificate to a client to convince them of the existence and finality of a transition within \sysname, with no further action or interaction within the system. If a checkpoint of finalized certificates is available, at an epoch boundary or otherwise, a bundle of evidence including the input objects and certificate, alongside a proof of inclusion of the certificate in the checkpoint is also a proof of finality.

%Authorities may use a periodic checkpointing mechanism to create collective checkpoints of finalized transactions, as well as the state of \sysname over time. A certificate with a quorum of stake over a checkpoint can be used by light clients to efficiently validate the recent state of objects and emitted events. A check pointing mechanism is necessary for committee reconfiguration between epochs. More frequent checkpoints are useful to light clients, and may also be used by authorities to compress their internal data structures as well as synchronize their state with other authorities more efficiently.

%\subsection{Full Replicas}
%\alberto{Explain here replicas (fullnodes). They do not process transactions (only certificates) and modify $\ownedlockdb$ db to detect conflicting certificates.}

%\subsection{Bridges}
%\george{Since we do not build first party bridges, I think we should eliminate this section to avoid any confusion.}
%Native support for light clients and shared objects managed by Byzantine agreement allows \sysname to support two-way bridges to other blockchains~\cite{DBLP:journals/iacr/McCorryBYS21}. The trust assumption of such bridges reflect the trust assumptions of \sysname and the other blockchain, and do not have to rely on trusted oracles or hardware if the other blockchain also supports light clients~\cite{ChatzigiannisBC21a}. \sysname provides the permission-less exhaustive access to state data required to support trust-minimized bridge architectures.

%Bridges are used to import an asset issued on another blockchain, to represent it and use it as a wrapped asset within the \sysname system.In such cases the asset is locked on a smart contract on the other blockchain; \sysname authorities use light client support to read it is locked, and materialize it as a wrapped asset owned by a user on \sysname. The asset may be transferred within \sysname, or be composed within other objects.
%Eventually, the wrapped asset can be unlocked and transferred back to a user on the native blockchain.

%Bridges can also allow assets issued on \sysname to be locked, and used as wrapped assets on other blockchains.
%In this case the asset is locked on \sysname, through a bridge represented as a shared object that maintains the bridge state. The smart contract on the other blockchain is provided with the proof the asset has been locked, using \sysname light client support; and materializes the object on the other blockchain as a wrapped \sysname object, that may be used within the other system.
%Eventually, the wrapped object on the other system can be destroyed, and the object on \sysname updated to reflect any changes of state or ownership, and unlocked.

%The semantics of bridged assets are of some importance to ensure wrapped assets are useful. Fungible assets bridged across blockchains can provide a richer wrapped representation that allows them to be divisible and transferable when wrapped. Non-fungible assets are not divisible, but only transferable. They may also support other operations that mutates their state in a controlled manner when wrapped, which may necessitate custom smart contract logic to be executed when they are bridged back and unwrapped. \sysname is flexible and allows smart contract authors to define such experiences, since bridges are just smart contracts implemented in Move rather than native \sysname concepts -- and therefore can be extended using the composability and safety guarantees Move provides.

\para{Rewards \& cryptoeconomics} \george{We can be a little more complete here?}
\sysname has a native token \systoken, with a fixed supply. \systoken is used to pay for gas, and is also be used as delegated stake on authorities within an epoch. The voting power of authorities within this epoch is a function of this delegated stake. At the end of the epoch fees collected through all transactions processed are distributed to authorities according to their contribution to the operation of \sysname, and in turn they share some of the fees as rewards to addresses that delegated stake to them.

\kostas{IMO if we have space in Appendix, we should mention a few concrete dapps that fit to either the single-owner model or shared-object or mixed (ie lotteries, price quotes). This will make it by far easier for reviewers to conceptualize why such a system can be useful (we have this already and happy to take that), I had the feeling while reading the paper that this is too important for justifying/visualizing the need for a more complex design + the mixed model has never been referenced either in fastpay paper or all of the BFT systems, because it's unique in Sui/Capy}



==> sections/600Discussion.tex <==
\section{Discussion}

==> sections/650Scaling.tex <==
\section{Scaling and Latency}
The \sysname system allows scaling though authorities devoting more resources, namely
CPUs, memory, network and storage within a machine or over multiple machines, to the 
processing of transactions. More resources lead to an increased ability to process 
transactions, leading to increased fees income to fund these resources. More resources 
also results in lower latency, as operations are performed without waiting for necessary resources 
to become available.

\vspace{3mm}
\noindent \textbf{Throughput.} To ensure that more resources result in increased capacity 
quasi-linearly, the \sysname design aggressively reduces bottlenecks and points 
of synchronization requiring global locks within authorities. Processing 
transactions is cleanly separated into two phases, namely (1) ensuring the
transaction has exclusive access to the owned or shared objects at a specific version,
and (2) then subsequently executing the transaction and committing its effects. 

Phase (1) requires a transaction acquiring distributed locks at the granularity of objects.
For owned objects this is performed trough a reliable broadcast primitive, that 
requires no global synchronization within the authority, and therefore can be 
scaled through sharding the management of locks across multiple machines by 
$\objectid$. For transactions involving shared objects sequencing is required using
a consensus protocol, which does impose a global order on these transactions 
and has the potential to be a bottleneck. However, recent advances on engineering 
high-throughput consensus protocols~\cite{narwhal} demonstrate that sequential 
execution is the bottleneck in state machine replication, not sequencing. In \sysname,
sequencing is only used to determine a version for the input shared object, namely 
incrementing an object version number and associating it with the transaction digest, 
rather than performing sequential execution.%
% \francois{This should articulate a practical thesis for why the burden of performing 2 broadcasts in order to submit a transaction is not significant (basically: network costs are shrinking, and network services will grow like wildfire, offering menial costs).}
% George says: we will do that when we have benchmarks, with evidence rather than 
% a deductive argument. Logic cannot be used to settle performance questions.

Phase (2) takes place when the version of all input objects is known to an authority
(and safely agreed across authorities) and involves execution of the Move transaction
and commitment of its effects. Once the version of input objects is known, execution can
take place completely in parallel. Move virtual machines on multiple cores or physical machines
read the versioned input objects, execute, and write the resulting objects
from and to stores. The consistency requirements on stores for objects and transactions 
(besides the order lock map) are very loose, allowing scalable distributed key-value stores 
to be used internally by each authority. Execution is idempotent, making even crashes 
or hardware failures on components handling execution easy to recover from. 

As a result, 
execution for transactions that are not causally related to each other can proceed in 
parallel. Smart contract designers may therefore design the data model of objects and 
operations within their contracts to take advantage of this parallelism.

Check-pointing and state commitments are computed off the critical transaction processing path 
to not block the handling of fresh transactions. These involve read operations 
on committed data rather than requiring computation and agreement before a 
transaction reaches finality. Therefore they do not affect the latency 
or throughput of processing new transactions, and can themselves be distributed across available 
resources.

Reads can benefit from very aggressive, and scalable caching. Authorities sign and make 
available all data that light clients require for reads, which may be served by distributed
stores as static data. Certificates act as roots of trust for their full causal history of
transactions and objects. State commitments further allow for the whole system to have regular 
global roots of trust for all state and transactions processed, at least every epoch or more 
frequently.

\vspace{3mm}
\noindent \textbf{Latency.} Smart contract designers are given the flexibility to control
the latency of operations they define, depending on whether they involve owned or shared
objects. Owned objects rely on a reliable broadcast before execution and commit, 
which requires two round trips to a quorum of authorities to reach finality. Operations 
involving shared objects, on the other hand, require a a consistent broadcast to create
a certificate, and then be processed within a consensus protocol, leading to increased 
latency (4 to 8 round trips to quorums as of~\cite{narwhal}). 


==> sections/700Conclusions.tex <==
\section{Conclusion}
\sysname is the first smart-contract platform that forgoes consensus for single-writer operations and only relies on consensus for settling multi-writer operations, combining the two modes securely.
%
We describe system aspects to achieve long-term stability and production-readiness that are typically overlooked by research prototypes. It proposes checkpointing transactions into a sequence after execution (for large categories of transactions) to reduce the need for agreement and latency, and shows how to safely reconfigure the system with minimal downtime.
%
\sysname is currently running in production as part of a major smart-contract platform.
\shortBragging

==> sections/750Simpler.tex <==
\section{V0 algorithms}
\alberto{Do not delete yet}

\alberto{It would be nice of the active state could be $O(n)$ in the number of objects rather than in the number of transactions. Let's see if we can do that here (reviewers may complain)}

\alberto{Explain how to cleanup the shared locks stores 'as we go' by swapping the checks \Cref{alg:line:shared-lock-check-1} and \Cref{alg:line:shared-lock-check-2}.}

\begin{algorithm}[t]
    \caption{Storage support (generic)}
    \label{alg:storage-support}
    \small
    \begin{algorithmic}[1]
        \Statex // Check whether the  certificate as already been executed.
        \Procedure{AlreadyExecuted}{\cert}
        \State $\transactiondigest = \txdigest{\cert}$
        \State $(\_, \esign) = \certdb_v[\transactiondigest]$
        \If{$\esign$}
        \Return $\esign$
        \EndIf
        \Return \textbf{None}
        \EndProcedure

        \Statex
        \Statex // All operations inside this functions are atomic.
        \Procedure{AtomicPersist}{$\cert, \esign, [\Obj_{out}]$}
        \State \Call{DeleteSharedLocks}{$\cert$} \Comment{Defined in \Cref{alg:storage-support-shared-objects}}
        \State $\transactiondigest = \txdigest{\cert}$
        \State $\certdb_v[\transactiondigest] = (\cert, \esign)$
        \For{$\Obj$ in $\Obj_{out}$}
        \State $\objectref = \oref{\Obj}$
        \State $\objdb_v[\objectref] = \Obj$
        \State $\syncdb_v[\objectref] = \transactiondigest$
        \EndFor
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{Storage support (shared objects)}
    \label{alg:storage-support-shared-objects}
    \small
    \begin{algorithmic}[1]
        \Statex // Assign locks to the shared-objects referenced by \cert.
        \Procedure{WriteSharedLocks}{$\cert$}
        \State $\transactiondigest = \txdigest{\cert}$
        \For{$\ObjID$ in $\txsharedinputs{\cert}$}
        \State $\Version = \nextsharedlockdb[\ObjID]$
        \State $\sharedlockdb[(\transactiondigest, \ObjID)] = \Version$
        \State $\nextsharedlockdb[\ObjID] = \Version + 1$
        \EndFor
        \EndProcedure

        \Statex
        \Statex // Cleanup the shared locks table.
        \Procedure{DeleteSharedLocks}{$\cert$}
        \State $\transactiondigest = \txdigest{\cert}$
        \For{$\ObjID$ in $\txsharedinputs{\cert}$}
        \State \textbf{delete} $\sharedlockdb[(\transactiondigest, \ObjID)]$
        \If{$!\objdb_v[\ObjID]$}\Comment{if the object does not exist}
        \State \textbf{delete} $\nextsharedlockdb[\ObjID]$
        \EndIf
        \EndFor
        \EndProcedure

        \Statex
        \Statex // Check whether all shared-objects referenced by \cert are locked.
        \Procedure{SharedLocksExist}{$\cert$}
        \State $\transactiondigest = \txdigest{\cert}$
        \For{$\ObjID$ in $\txsharedinputs{\cert}$}
        \If{$!\sharedlockdb[(\transactiondigest, \ObjID)]$}
        \State \Return false \Comment{lock not found}
        \EndIf
        \EndFor
        \State \Return true
        \EndProcedure

        \Statex
        \Statex // Ensure that \cert is the next certificate scheduled for execution.
        \Procedure{CheckSharedLocks}{$\cert$}
        \State $\transactiondigest = \txdigest{\cert}$
        \For{$\ObjID$ in $\txsharedinputs{\cert}$}
        \State $\Obj = \objdb_v[\ObjID]$
        \State $\Version = \version{\Obj}$
        \If{$\sharedlockdb[(\transactiondigest, \ObjID)] \neq \Version$}
        \State \Return false
        \EndIf
        \EndFor
        \State \Return true
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{Process transaction}
    \label{alg:process-tx}
    \small
    \begin{algorithmic}[1]
        \Statex // Executed upon receiving a transaction from a user.
        \Statex // Many tasks can call this function.
        \Procedure{ProcessTx}{$\transaction$}
        \If{$\txepoch{\transaction} \neq \epoch$} \Return Error \EndIf
        \State [\object] = \Call{LoadObjects}{$\txinputs{\transaction}$}  \Comment{Error if objects not found}
        \If{!$\txvalid{\transaction, [\object]}$} \Return Error \EndIf
        \State
        \State // Ensure all objects exist.
        \For{$\objectref$ in $\txinputs{\transaction}$}
        \If{$!\objdb_v[\objectref]$}
        \State \Return Error
        \EndIf
        \EndFor
        \For{$\objectid$ in $\txreadonly{\transaction} + \txsharedinputs{\transaction}$}
        \State $\objectref = (\objectid, *, *)$ \Comment{Version and digest unspecified}
        \If{$!\objdb_v[\objectref]$}
        \State \Return Error
        \EndIf
        \EndFor
        \State
        \State // Lock all owned-objects.
        \State $\txsign = \sign{\transaction}$
        \For{$\objectref$ in $\txinputs{\transaction}$}
        \If{$\txdb_v[\objectref] == \textsf{None}$}
        \State $\txdb_v[\objectref] = \txsign$
        \ElsIf{$\txdb_v[\objectref] \neq \txsign$}
        \State \Return Error
        \EndIf
        \EndFor
        \State
        \State \Return \txsign
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{Process certificate}
    \label{alg:process-cert}
    \small
    \begin{algorithmic}[1]
        \Require Input \cert is signed by a quorum

        \Statex
        \Statex // Executed upon receiving a certificate from a user.
        \Statex // Many tasks can call this function.
        \Procedure{ProcessCert}{$\cert$}
        \If{$\txepoch{\cert} \neq \epoch$} \Return Error \EndIf
        \State
        \State // Check wether the transaction has already been executed.
        \State $\esign = \Call{AlreadyExecuted}{\cert}$
        \If{$\esign \neq$ \textbf{None}}
        \State \Return $\esign$ \Comment{Certificarte already executed}
        \EndIf
        \State
        \State // Load objects from store, return error if an object is missing.
        \State [$\object_o$] = \Call{LoadObjects}{$\txinputs{\cert}$}
        \State [$\object_{s}$] = \Call{LoadObjects}{$\txsharedinputs{\cert}$}
        \State
        \State // Check the objects locks.
        \For{$(\objectref, \object)$ in \textbf{zip}($\txinputs{\transaction}, [\Object_o])$}
        \If{$\version{\objectref} \neq \version{\Obj}$}
        \State \Return Error
        \EndIf
        \EndFor
        \If{!\Call{SharedLocksExist}{$\cert$}}
        \State \Call{ForwardToConsensus}{$\cert$} \Comment{Sequence the certificates}
        \State \Return
        \EndIf
        \If{!\Call{CheckSharedLocks}{$\cert$}} \Return Error \EndIf
        \State
        \State // Execute the certificate.
        \State $(\esign, [\Obj_{out}]) = \txexec{\cert, [\object_{o}], [\object_{s}]}$
        \State \Call{AtomicPersist}{$\cert, \esign, [\Obj_{out}]$}
        \EndProcedure

        \Statex
        \Statex // Executed upon receiving a certificate from consensus.
        \Statex // This function must be called by a single task.
        \Procedure{AssignSharedLocks}{$\cert$}
        \State exist = \Call{SharedLocksExist}{$\cert$}
        \If{$\Call{AlreadyExecuted}{\cert}$} \Return \EndIf
        \If{!exist} \Call{WriteSharedLocks}{$\cert$} \EndIf
        \EndProcedure
    \end{algorithmic}
\end{algorithm}



==> sections/800Specification.tex <==
\section{Specification} \label{sec:specification}
This section provides a semi-formal specification for the validation and execution of FastX transactions. We use the term "validating" to describe the authority-side processing performed on a $\transaction$, and "executing" to describe the authority-side processing performed on a $\cert$. We first describe the steps common to processing any transaction or certificate, then describe steps specific to the payload (i.e., $\mathsf{Call}$ or $\Publish$) of the transaction/certificate.

\begin{figure}
  \begin{tabular}{|ll|}
  \hline
  \textbf{Addresses and ID's} & \\
  \hline
  $\Authenticator =$ & $\mathsf{PubKey} \uplus \objectid \uplus \ldots$ \\
  $\AccountAddress =$ & $Com(\Authenticator)$ \\
  $\transactiondigest =$ & $Com(\transaction)$ \\
  $\objectid =$ & $Com(\transactiondigest \times \mathbb{N})$ \\
  $\ModuleID =$ & $\objectid \times \ModuleName$ \\
  \hline
  \textbf{Types and Kinds} & \\
  \hline
  $\GroundType =$ & $\set{\texttt{address}, \texttt{bool}, \texttt{u64}, \texttt{bytes}}$ \\
  $\StructType =$ & $\ModuleID \times \StructName$ \\
  $\StoreableType =$ & $\GroundType \uplus \StructType$ \\
  $\MutabilityQual =$ & $\set{\texttt{mut}, \texttt{immut}}$ \\
  $\ReferenceType =$ & $\StoreableType \times \MutabilityQual$ \\
  $\Type =$ & $\mathsf{ReferenceType} \uplus \StoreableType$ \\
  $\Kind =$ & $\set{\texttt{key}, \texttt{store}, \texttt{copy}, \texttt{drop}}$ \\
  \hline
  \textbf{Values and State} & \\
  \hline
  $\PrimValue=$ & $\AccountAddress \uplus \mathsf{Bytes} \uplus \mathbb{B} \uplus \mathbb{N}$ \\
  $\Struct =$ & $\FieldName \pfun \StoreableValue$ \\
  $\StoreableValue =$ & $\Struct \uplus \PrimValue$ \\
  $\Reference =$ & $\Var \times \seq{\FieldName}$ \\
  $\Value =$ & $\StoreableValue \uplus \Reference$ \\
  $\LocalEnv =$ & $\Var \pfun \Value$ \\
  $\CallStackFrame =$ & $\ProcID \times \PC \times \LocalEnv$ \\
  $\CallStack =$ & $\seq{\CallStackFrame}$ \\
  $\OperandStack =$ & $\seq{\Value}$ \\
  $\textsf{State} =$ & $\CallStack \times \OperandStack$ \\
  \hline
  \textbf{Modules} & \\
  \hline
  $\Module =$ & $\ModuleID \times (\StructName \pfun \StructDecl)$ \\
  & $\times (\ProcName \pfun \ProcDecl) \times \seq{\ModuleID}$ \\
  $\StructDecl =$ & $\seq{\Kind} \times(\FieldName \pfun \StoreableType)$ \\
  $\ProcDecl$ = & $\seq{\seq{\Kind}} \times \seq{\Type} \times \seq{\Type} \times \seq{\Instruction}$ \\
  $\Instruction=$ & $\ldots$ \\
    \hline
     \textbf{Events} & \\
  \hline
  $\Transfer =$ & $\ObjID \times \Struct \times \StructType \times \AccountAddress$ \\
  $\Freeze =$ & $\ObjID \times \StructType \times \Struct$ \\
  $\Event =$ & $\Transfer \uplus \Freeze \uplus \ldots$ \\

  \hline
  \end{tabular}

  \caption{Semantic definitions for the Move-powered core of FastX.}
  \end{figure}

\begin{figure}
\begin{tabular}{|ll|}\hline
\textbf{Objects} & \\
  \hline
  $\mathsf{MoveObjType} =$ & $\StructType \times \MutabilityQual$ \\
  $\mathsf{ObjType} =$ & $\mathsf{MoveObjType} \uplus \{ \texttt{code} \}$ \\
  $\mathsf{ObjData} =$ & $\Struct \uplus \Module$ \\
  $\Object =$ & $\mathsf{ObjData} \times \mathsf{ObjType} \times \AccountAddress \times \transactiondigest$  \\
  & $\times \Version$ \\
    \hline
  \textbf{Transactions} & \\
  \hline
  $\ObjRef=$ & $\objectid \times \transactiondigest \times Com(\Object)$ \\
  $\textsf{GasFee} =$ & $\ObjRef$ \\
  $\textsf{CallTarget}=$ & $\ObjRef \times \ProcName$ \\
  $\textsf{Call} =$ & $\textsf{CallTarget} \times \seq{\StoreableType} \times \seq{\ObjRef}$ \\
  & $\times \seq{\PrimValue} \times \textsf{GasBudget}$ \\
  $\textsf{Publish} =$ & $\Module \times \seq{\ObjRef}$ \\
  $\UserSig =$ & $\AccountAddress \times \Authenticator \times \Sig$ \\
  $\mathsf{AuthorityName} =$ & $\mathsf{PublicKey}$ \\
  $\AuthoritySig =$ & $\mathsf{AuthorityName} \times \Sig$ \\
  $\mathsf{TxMsg} =$ & $(\textsf{Call} \uplus \textsf{Publish}) \times \textsf{GasFee} \times \textsf{GasPrice}$ \\ 
  & $\times \textsf{EpochID}$ \\
  $\transaction =$ & $\mathsf{TxMsg} \times \UserSig$ \\
  $\textsf{SignedTx} =$ & $\transaction \times \AuthoritySig$ \\
  $\cert =$ & $\transaction \times \seq{\AuthoritySig}$ \\
\hline
\textbf{Stores} & \\
\hline
 $\mathsf{LockMap} =$ & $\ObjRef \pfun \transaction_{\bot}$ \\
 $\mathsf{CertMap} =$ & $\transactiondigest \pfun \transaction \times \cert$ \\
 $\mathsf{ObjMap} =$ & $\objectid \pfun \Object_{\bot}$ \\
 $\mathsf{SyncMap} =$ & $\objectid \times \transactiondigest \pfun \cert$ \\

 \hline
\end{tabular}
  
\caption{Semantic definitions for the FastX transactions and persistent storage}
\end{figure}



\subsection{Common Processing}
\paragraph{Transaction Prologue}
The following checks are performed on all $\transaction$'s. The authority should authenticate the sender of the message and check that its mutable input objects have not previously been used. In detail:
\begin{enumerate}
    \item $\transaction.\UserSig.\Sig$ is cryptographically valid signature on the message $\transaction.\mathsf{TxMsg}$ w.r.t $\transaction.\UserSig.\Authenticator$
    \item The transaction sender \\  $\transaction.\UserSig.\AccountAddress$ matches $Com(\UserSig.\Authenticator)$
    \item The $\EpochID$ matches the current epoch
    \item For all $\ObjRef$ inputs, $\objectid$ is unique (i.e., no duplicate inputs)
    \item $\ObjMap[\objectid]$ exists for all $\ObjRef$ inputs
    \item $\ObjRef.\transactiondigest = \ObjMap[\ObjRef.\objectid].\transactiondigest$ for all $\ObjRef$'s (i.e., each object input correctly points to the transaction that created or last mutated it)
    \item $Com(\Object)$ matches $\ObjMap[\ObjRef.\objectid]$ for all $\ObjRef$ inputs, (i.e., each input commits to the correct value of its corresponding object in persistent storage)
    \item For all mutable $\ObjRef$ inputs, $\LockMap[\ObjRef]$ exists and either is not set, or is set to exactly the same transaction (i.e., the authority is not waiting on confirmation of a different transaction accepting any of these objects as input)
\end{enumerate}

\paragraph{Transaction Epilogue}
If all of these checks pass, the authority should:
\begin{enumerate}
    \item Set $\LockMap[\ObjRef] = \transaction$ for all mutable $\ObjRef$ inputs. TODO: explain how to determine input mutability--anything passed by value or as a mutable reference. Immutable objects, or immutable references to mutable objects don't count as mutable
    \item Sign the message to create an $\AuthoritySig$ and return a $\SignedTx$ to the user.
\end{enumerate}

\paragraph{Certificate Prologue}
The following checks should be performed prior to processing any $\cert$:
\begin{enumerate}
    \item For each $\AuthoritySig$ in the certificate, $\cert.\AuthoritySig.\Sig$ is cryptographically valid signature on the message $\transaction$ w.r.t public key $\cert.\AuthoritySig.\mathsf{AuthorityName}$
    \item $\cert.\transaction.\EpochID$ matches the current epoch
    \item $\AuthoritySig.\mathsf{AuthorityName}$ is an authority in the current epoch
    \item $|\seq{\AuthoritySig}| \geq N - F$, where $N$ is the number of authorities in the current epoch and $F$ the number of failures tolerated (i.e., the certificate has signatures from a quorum of authorities. Note that $N > 3F$.)
    \item $\LockMap[\ObjRef]$ exists for each mutable $\ObjRef$ input to the transaction TODO: this is needed to prevent out of order execution. but we could consider relaxing this if we are comfortable with out of order exec.
\end{enumerate}

\paragraph{Certificate Epilogue}
The following actions should be performed at the conclusion of processing any $\cert$:
\begin{enumerate}
    \item Update the value of $\ObjMap[\GasFee.\ObjID].\ObjData$ to the gas used during execution multiplied by $\GasPrice$ (i.e., pay for gas)
    \item Increment $\ObjMap[\GasFee.\ObjID].\Version$ (i.e., reflect that the gas object has been mutated via paying for gas)
    \item Update $\ObjMap[\GasFee.\ObjID].\transactiondigest$ to the digest of the current transaction (i.e., reflect that this transaction mutated the gas fee object)
    \item Delete entry $\LockMap[\ObjRef]$ for all mutable $\ObjRef$ inputs (whether it is set of not).
    \item Update $\CertMap$ with the current $\transaction$ and $\cert$
\end{enumerate}

\subsection{Processing a $\mathsf{Call}$}
\paragraph{$\mathsf{Call}$ Transaction Prologue}
For a $\transaction$ containing a $\mathsf{Call}$ payload, the authority should perform these additional validation checks as part of the prologue: 
\begin{enumerate}
    \item For the $\GasFee$, the value of $\ObjMap[\GasFee.\objectid].\ObjData$ object is greater than or equal to $\GasBudget * \GasPrice$ (i.e., the fee is sufficient) TODO: explain how to extract the value
\end{enumerate}

\paragraph{$\mathsf{Call}$ Certificate Prologue}
The input is a $\cert$ containing a $\mathsf{Call}$ payload. In addition to performing the certificate prologue described above, the authority should type-check the call:

\begin{enumerate}
    \item $\ObjMap[\CallTarget.\ObjID].\ObjType$ is \texttt{code}
    \item $\CallTarget.\ProcName$ is a public function declared by this module
    \item The arity of the function is $|\seq{\ObjRef}| + |\seq{\PrimValue}| + 1$. TODO: explain the +1--for a special transaction-local \texttt{TxContext} object constructed by the adapter using the $\transactiondigest$ and sender address
    \item For all $\ObjRef$'s, the type of the $i$th input \\ $\ObjMap[\ObjID_i].\ObjType.\StructType$ is equal to the reference-stripped type of the $i$th parameter in the type signature of the function (i.e., the transaction inputs are well-typed w.r.t the function). TODO: explain reference stripping
    \item For all mutable $\ObjRef$ inputs, the type of the $i$th input \\ $\ObjMap[\ObjID_i].\ObjType.\MutabilityQual$ is \texttt{mut} (i.e., the transaction does not attempt to mutate immutable objects)
    \item The function has no return types
    \item For all$\seq{\PrimValue}$ arguments, the $i$th argument can be deserialized using to the $i + |\seq{\ObjRef}|$th parameter type (i.e., each primitive value argument is well-typed w.r.t the function signature).
    \item For each $\StructType$ argument in the type arguments \\ $\seq{\StoreableType}$, the entry $\ObjMap[\StructType.\ModuleID.\ObjID]$ exists (i.e., the type arguments refer to valid types)
\end{enumerate}

If these checks pass, the authority should run the code embedded in the payload. In detail:
\begin{enumerate}
    \item Bind the type arguments in $\seq{\StoreableType}$ to the type parameters of the function
    \item Create arguments by concatenating $\Struct$'s extracted from the object inputs inputs to the $\PrimValue$ inputs. TODO: more details on how this works, particularly with reference inputs
    \item Bind these arguments to the parameters of the $\ProcDecl$ and execute the entrypoint using the Move VM
\end{enumerate}

\paragraph{$\mathsf{Call}$ Certificate Epilogue}
Execution terminates with the amount of gas used and a status code indicating whether execution concluded successfully or \emph{aborted}. If execution succeeds, the outputs are (A) changes to the mutable input $\Struct$'s that were passed by reference and (B) a log of events emitted by execution. The events in (B) may include distinguished $\Transfer$ and $\Freeze$ events with special interpretations, as well as user-defined events.

In the case of a successful execution, the authority should:

\begin{enumerate}
    \item Update the $\ObjData$ of each object in (A) in $\ObjMap$. This reflects the modifications made to objects that were passed to the entrypoint via a mutable reference.
    \item For each object passed by value to the entrypoint: create a temporary map $\mathsf{Inputs}: \ObjID \pfun \Object$ reflecting the value of each object before the function was called. Delete each object that was passed by value to the entrypoint by writing $\ObjMap[\ObjRef.\ObjID] = \bot$ for each input $\ObjRef$ passed by value
    \item For each $\Transfer$ event in (B): if the $\ObjID$ \emph{is not} in $\mathsf{Inputs}$, create a new $\Object$ with $\ObjData$ containing the $\Struct$ from the event, $\ObjType$ as the $\StructType$ from the event plus $\texttt{mut}$ as a $\MutabilityQual$, $\AccountAddress$ as the address from the event, $\transactiondigest$ as the digest of the current transaction, and $\Version$ 0. (i.e., transfer an object created by this transaction)
    \item For each $\Freeze$ event in (B): if the $\ObjID$ \emph{is not} in $\mathsf{Inputs}$, create a new $\Object$ with $\ObjData$ containing the $\Struct$ from the event plus $\texttt{immut}$ as a $\MutabilityQual$,, $\ObjType$ as the $\StructType$ from the event, $\AccountAddress$ as $\UserSig.\AccountAddress$, $\transactiondigest$ as the digest of the current transaction, and $\Version$ 0. (i.e., freeze an object created by this transaction)
    \item For each $\Transfer$ event in (B): if the $\ObjID$ \emph{is} in $\mathsf{Inputs}$, update $\mathsf{Inputs}[\ObjID].\ObjData$ to the $\Struct$ from the event, and $\mathsf{Inputs}[\ObjID].\AccountAddress$ to the $\AccountAddress$ (i.e., transfer an object passed by value to this transaction). Update $\ObjMap[\ObjID]$ with $\mathsf{Inputs}[\ObjID]$ for each of these objects.
    \item For each $\Freeze$ event in (B): if the $\ObjID$ \emph{is} in $\mathsf{Inputs}$, update $\mathsf{Inputs}[\ObjID].\ObjData$ to the $\Struct$ from the event,  and $\mathsf{Inputs}[\ObjID].\ObjType.\MutabilityQual$ to $\texttt{immut}$. (i.e., freeze an object passed by value to this transaction). Update $\ObjMap[\ObjID]$ with $\mathsf{Inputs}[\ObjID]$ for each of these objects.
    \item For each $\ObjID$ in $\mathsf{Inputs}$ that did not appear in a $\Freeze$ or $\Transfer$ event, delete the object by updating $\ObjMap[\ObjID] = \bot$ (i.e., delete inputs passed by value that were neither transferred nor frozen) TODO: should we leave the $\Object$ but set its $\ObjData$ to $\bot$?
    \item Increment the $\Version$ of each object in (A) and the transferred/frozen objects that were not freshly created
    \item Update the $\transactiondigest$ of each object in (A) and the transferred/frozen objects to the digest of the current transaction
    \item For each $\Transfer$ event in (B) and each mutable object in (A): update $\LockMap[\ObjID \times \transactiondigest] = \transaction$, where $\transaction$ is the current transaction and $\transactiondigest$ is the digest of the current transaction (i.e., create a lock for each new mutable $\ObjRef$).
    
    \item TODO: describe processing of use-defined events
\end{enumerate}

In the case of either successful execution, aborted execution, or failed typechecking of the function, the authority should perform the transaction epilogue described above. TODO: say what gas used should be if typechecking fails

\subsection{Processing a $\Publish$}
\paragraph{$\Publish$ Transaction Prologue}
For a $\transaction$ containing a $\Publish$ payload, the authority should perform these validation checks in addition to the transaction prologue described above: 

\begin{enumerate}
    \item For the $\GasFee$, the value of $\ObjMap[\objectid].\ObjData$ object is greater than or equal to the $\GasPrice$ multiplied by the size of the module in bytes (i.e., the fee is sufficient) TODO: may want a flat fee or additional multiplier
    \item $\ObjMap[\ObjRef.\ObjID].\ObjType$ is \texttt{code} for each $\ObjRef$ included in the payload (i.e., each input is a module)
    \item The list $\seq{\ObjRef.\ObjID].\ObjData.\ModuleID}$ for each $\ObjRef$ included in the payload is equal to $\Module.\seq{\ModuleID}$ (i.e., the declared dependencies of the module exactly match the $\ObjRef$'s passed as input
\end{enumerate}

\paragraph{$\Publish$ Certificate Prologue}
The input is a $\cert$ containing a $\Publish$ payload. The authority should first verify the module:

\begin{enumerate}
\item Run the Move bytecode verifier on the $\Module$ in the payload
\item Run the Move linker on the $\Module$ and its dependencies (i.e., ensure that the handles in the current module match their declarations in its dependencies)
\item Run the FastX-specific bytecode verifier passes on the $\Module$ in the payload
\item Check that the $\ObjID$ in the $\Module$ is 00...0
\end{enumerate}

\paragraph{$\Publish$ Certificate Epilogue}
If verification passes, the authority should publish the module as an object:

\begin{enumerate}
\item Create a fresh $\ObjID$ for the module from the $\transactiondigest$ of the current transaction and an $\mathsf{OutputIndex}$ of 0
\item Overwrite the existing $\ObjID$ of the $\Module$ with this fresh ID.
\item Create an $\Object$ containing this modified $\Module$, type \texttt{code}, the $\AccountAddress$ of the transaction sender, $\transactiondigest$ of the current transaction, and $\Version$ 0. Insert this object into $\ObjMap[\ObjID]$.
\end{enumerate}

In the case of either successful verification or failed verification, the authority should perform the transaction epilogue described above.


==> sections/950Deletion.tex <==
\section{Generalizing Objects Deletion} \label{sec:elegant-deletion}
As explained in \Cref{sec:objects-deletion}, it is a challenging to allow deletion of \sysname objects without opening the system to replay attacks.
%
However, unlike sharded blockchains that face the same problem during cross-shard transactions~\cite{byzcuit}, \sysname has an advantage. The same set of nodes runs both paths, hence we can employ quorum-based algorithms to prevent the replay without any extra memory costs.
Unfortunately, such solutions would be prohibitive as they require an $O(n^2)$ total message complexity for every object and every potential message that can be replayed. We present the protocol for completeness but do not implement it for \sysname; \sysname instead runs the protocol described in \Cref{sec:objects-deletion}.
%
The protocol works in three steps:
\begin{enumerate}
    \item Initialize: The object is created on the consensus-less path and an effect certificate logs the $2f+1$ parties that should have created it in their local state
    \item Create: A transaction using the shared object is submitted through consensus together with the effects certificate of creation. The $2f+1$ parties ($f+1$ honest) have already created the object so they simply continue. For the $f$ parties that did not participate, they need to know whether this is a replay attack or not. To this end, they query the parties that signed the effects certificate.
    \item Verify:  If the transaction is indeed the first to access the created object then $f+1$ honest parties will reply affirmatively otherwise they will reply negatively. As a result, the slow parties are bound to act as per the protocol without any need for extra memory.
\end{enumerate}

%\lef{Open question if we can somehow piggyback these acks/nacks on state commitments. Unfortunately due to batching this seems to create a deadlock scenario if two replays happen in the same batch}
